Fairness Shields: Safeguarding against Biased Decision Makers

As AI-based decision-makers increasingly influence human lives, it is a growing concern that their decisions are often unfair or biased with respect to people's sensitive attributes, such as gender and race. Most existing bias prevention measures provide probabilistic fairness guarantees in the long run, and it is possible that the decisions are biased on specific instances of short decision sequences. We introduce fairness shielding, where a symbolic decision-maker -- the fairness shield -- continuously monitors the sequence of decisions of another deployed black-box decision-maker, and makes interventions so that a given fairness criterion is met while the total intervention costs are minimized. We present four different algorithms for computing fairness shields, among which one guarantees fairness over fixed horizons, and three guarantee fairness periodically after fixed intervals. Given a distribution over future decisions and their intervention costs, our algorithms solve different instances of bounded-horizon optimal control problems with different levels of computational costs and optimality guarantees. Our empirical evaluation demonstrates the effectiveness of these shields in ensuring fairness while maintaining cost efficiency across various scenarios.

==> 40_unbounded.tex <==
\todo{Add a remark that naive will work with high probability, and in fact, experimentally works quite well. Question: is it true that with probability one, in a large enough number of time horizon, the biased cases will appear?}

The na\"ive approach to solve the periodic fairness-shield synthesis problem would be to reuse the shield designed for time horizon $T$ at each period.
This approach does not offer guarantees in terms of DP. 
In particular, in Fig.~\ref{fig:counter-example-periodic-naive} we show how
for a given horizon $T$, there exist traces $\tau_1, \tau_2$, 
such that $\DP(\tau_1) = \DP(\tau_2) = 0$, 
and $\DP(\tau_1\tau_2) = 1-2/T$, which grows arbitrarily close to $1$ with $T$.

\begin{figure}
    \centering
    \begin{tabular}{l | c c c c | c}
          & $n_a$ & $n_{a1}$ & $n_b$ & $n_{b1}$ & $\DP$   \\
          \hline
         $\tau_1$ & $1$ & $0$ & $T-1$ & $0$ & $0$\\
         $\tau_2$ & $T-1$ & $T-1$ & $1$ & $1$ & $0$ \\
         \hline
         $\tau_1\tau_2$ & $T$ & $T-1$ & $T$ & $1$  & $1-2/T$
    \end{tabular}
    \caption{Counter-example showing that the na\"ive repeated application of the bounded-horizon fairness-shield will not give us a periodic fairness-shield. \todo{Fill in the table}}
    \label{fig:counter-example-periodic-naive}
\end{figure}



In the following, we present two solutions for the periodic fairness-shield synthesis problem:
The first one is a \emph{dynamic} approach where the shield is re-computed at the beginning of each time period, where the re-computation accounts for the aggregated statistics in the past time periods.
The second one is a \emph{static} approach where the shield is computed only once for the horizon length $T$ but with a stricter constraint than merely satisfying the DP condition.
While the dynamic approach provides the optimal solution for Prob.~\ref{prob:unbounded}, it is computationally more expensive (because the shield needs to be recomputed repeatedly).
In contrast, the static approach produces a shield that is still fair but possibly incurs a larger cost, and has the benefit that it needs to be computed just once.

The dynamic shielding approach is based on the repeated calls to a sub-procedure that we refer to as the inductive shielding, which is presented in the following.


\subsection{Inductive Shielding: A Detour}
\todo{The name is a placeholder. I am not a big fan of ``buffered'' because it does not convey the intuition.}

Given a trace $\tau$ of arbitrary length such that $\DP(\tau)\leq \kappa$, define $\sShieldFeas^{t,\tau}$ as the set of shields over time $t$ such that for every feasible extension $\tau'\in (\aX\times\aY)^t$ of $\tau$, $\DP(\tau\tau') \leq \kappa$.
Formally,
% \begin{multline*}
%     \sShieldFeas^{t,\tau} \coloneqq \set{ \sshield\in\sShield \mid \forall \tau'\in (\aX\times\aY)^t\;.\; \\
%     \prob(\tau';P_\sagent,\sshield) > 0 \implies \DP(\tau\tau') \leq \kappa}.
% \end{multline*}

\[
\sShieldFeas^{t,\tau} \coloneqq \set{ \sshield\in\sShield \mid \forall \tau'\in \Trfeas^{t\mid\tau}_{\sagent,\sshield} \;.\; \DP(\tau\tau') \leq \kappa}.
\]



We refer to the elements in $\sShieldFeas^{t,\tau}$ as inductive fairness-shields with respect to $\tau$.
\FC{In this definition, I did not add $\kappa$ to the subscript of $\sShieldFeas$ to ease the notation, I think it should be clear by context.}

% In the dynamic approach, we solve the following sub-problem at the beginning of each new time period.



\begin{problem}[Inductive fairness-shield synthesis]
    Let $P_\sagent\in \distrset(\aX)$ be a given joint distribution of sampling individuals and the output of the agent $\sagent$, $\kappa>0$ be a given DP threshold, and $T>0$ be the time period.
    For every given past trace $\tau$ of arbitrary length, compute an inductive fairness-shield $\sshield^*$ with respect to $\tau$ over time $T$ that also minimizes the expected cost, i.e., 
    \begin{align*}
        \sshield^* \coloneqq \arg\min_{\sshield\in\sShieldFeas^{T,\tau}} \expe[\cost;P_\sagent,\sshield,T].
    \end{align*}
\end{problem}

For a given past trace $\tau$, suppose $\ol{n}_a,\ol{n}_{a1},\ol{n}_b,\ol{n}_{b1}$ are the respective counter values for $\tau$.
The inductive fairness-shield with respect to $\tau$ can be computed by finding the optimal policy in the abstract MDP from Def.~\ref{def:abstract mdp} with the following slight modification: the cost function $\costmdp$ is now defined in a way such that
for every transition $\mathit{tr}=((\cdot,\cdot,\cdot,\cdot,\cX=(\cdot,r,c)),\cY,(n_a',n_{a1}',n_b',n_{b1}'))\in \Tran$,
\begin{itemize}
    \item If $n_a'+n_b'<T$ (the horizon has not been reached yet), then $C(\mathit{tr})$ is as defined in Def.~\ref{def:abstract mdp}.
    \item If $n_a'+n_b'=T$ (the horizon has been reached), then $C(\mathit{tr})=\infty$ if (the empirical DP, measured from the beginning of $\tau$, is violated):
    \[
        \DP(\ol{n}_a+n_a',\ol{n}_{a1}+n_{a1}',\ol{n}_b+n_b',\ol{n}_{b1}+n_{b1}') > \kappa,
    \]
    and $C(\mathit{tr})=0$ otherwise.
\end{itemize}

The following claim follows as a corollary of Thm.~\ref{thm:bounded-horizon shield synthesis}.
\begin{corollary}
    The inductive fairness-shield synthesis problem can be solved in $\mathcal{O}(T^4\cdot |\aX|)$-time.
\end{corollary}

\subsection{Dynamic Shielding}

The dynamic shielding problem can be solved by repeatedly solving the inductive shielding problem as a subroutine.
The procedure is summarized in the following.

\begin{enumerate}
    \item Compute the bounded-horizon cost-optimal fairness shield $\sshield^1$ over time $T$.
    Apply $\sshield^1$ up to time $T$.
    Let the generated trace be $\tau^1\in (\aX\times\aY)^T$.
    \item Repeat Step~\eqref{step:c} for $k=1,2,\ldots$.
    \item \label{step:c} Suppose $\tau^1\ldots\tau^k\in (\aX\times\aY)^{kT}$ is the trace generated up to time $kT$.
    Compute the inductive fairness-shield $\sshield^{k+1}$ with respect to $\tau^1\ldots\tau^k$.
    Apply $\sshield^{k+1}$ up to time $(k+1)T$.
    Let the generated trace in this segment be $\tau^{k+1}\in (\aX\times\aY)^T$.
\end{enumerate}

It can be easily verified that the resulting sequence of shields $\sshield^1\sshield^2\ldots$ is a periodic fairness-shield as sought in Prob.~\ref{prob:unbounded}.
\todo{Define concatenation of shields.}
The dynamic shielding approach is intuitive from the practical point of view: 
If a bank wants to maintain fairness at the end of each quarter starting from the beginning of year, it needs to recompute its policy by accounting for its decisions in the past quarters.
The drawback of the dynamic approach is that we need to keep computing the inductive shield repeatedly, which may turn out to be impractical in some applications.


\subsection{Static Shielding}

Static shielding eliminates the expensive period-wise re-computation step of dynamic shielding by computing one bounded-horizon shield over the period $T$ but with a more conservative goal than the fairness requirement of Prob.~\ref{prob:bounded}.
In particular static shielding will enforce a bound on the acceptance rates of each group. 
Given a trace $\tau = (g_1,\cdot,\cdot,y_1),\ldots,(g_t,\cdot,\cdot,y_t)\in (\aX\times\aY)^t$, the acceptance rate of group $g$ is 
$\AccRate{g}{\tau} = \frac{\sum_i \indicator{y_i=1\land g_i=g}}{\sum_i\indicator{g_i=g}}$.


For a given $t$, define $\sShieldFeasBounded^{t}$ as the set of every shield which guarantees that the acceptance rates of the two groups remain within the bounds $l$ and $u$.
Formally,
\begin{multline*}
    \sShieldFeasBounded^t \coloneqq \set{\sshield\in\sShield \mid \forall \tau \in \Trfeas^t_{\sagent, \sshield} \;.\; 
    \forall g\in \set{a,b}\;.\; \\
    l\leq \AccRate{g}{\tau} \leq u }.
\end{multline*}


Note that $\sShieldFeasBounded^t \subset \sShieldFeas^{t, \kappa}$ for $\kappa = u -l$.



% \vspace{2cm}
% In particular, static shielding requires the following assumption.
% \begin{assumption}\label{assump:bounds for static}
%     We are given a pair of fractions $l,u\in (0,1)$ such that $u-l = \kappa$, where $\kappa$ is the DP threshold.
% \end{assumption}


\begin{problem}[Static fairness-shield synthesis]\label{prob:static}
    Let $P_\sagent\in \distrset(\aX)$ be a given joint distribution of sampling individuals and the output of the agent $\sagent$, and let 
    $0 \leq l < u \leq 1$ be bounds on the acceptance rates.
    For every given time horizon $T>0$, compute a fairness-shield $\sshield^*$ over time $T$ that minimizes the expected cost after time $T$, i.e., 
    \begin{align*}
        \sshield^* \coloneqq \arg\min_{\sshield\in\sShieldFeasBounded^T} \expe[\cost;P_\sagent,\sshield,T].
    \end{align*}
\end{problem}
\todo{Use different notation for the different types of shields, instead of all of them being $\sshield^*$.}

The static fairness-shield can be computed by finding the optimal policy in the abstract MDP from Def.~\ref{def:abstract mdp} with the following slight modification: the cost function $\costmdp$ is now defined in a way such that
for every transition $\mathit{tr}=((\cdot,\cdot,\cdot,\cdot,\cX=(\cdot,r,c)),\cY,(n_a',n_{a1}',n_b',n_{b1}'))\in \Tran$,
\begin{itemize}
    \item If $n_a'+n_b'<T$ (the horizon has not been reached yet), then $C(\mathit{tr})$ is as defined in Def.~\ref{def:abstract mdp}.
    \item If $n_a'+n_b'=T$ (the horizon has been reached), then $C(\mathit{tr})=\infty$ if the acceptance rate of either of the groups is outside the range $[l,u]$:
    \[
        \exists g\in \set{a,b}\;.\; \frac{n_{g1}'}{n_g'}\notin [l, u],
    \]
    and $C(\mathit{tr})=0$ otherwise.
\end{itemize}

The following claim follows as a corollary of Thm.~\ref{thm:bounded-horizon shield synthesis}.
\begin{corollary}
    The static fairness-shield synthesis problem can be solved in $\mathcal{O}(T^4\cdot |\aX|)$-time.
\end{corollary}

The static fairness-shield can be used as is in every period to obtain a fairness-shield with respect to the DP criteria, though the optimality criterion in Prob.~\ref{prob:unbounded} may be violated.

\begin{theorem}
    Let $P_\sagent\in \distrset(\aX)$ be a given joint distribution of sampling individuals and the output of the agent $\sagent$, and let 
    $0 \leq l < u \leq 1$ be bounds on the acceptance rates.
%
    If $\sshield\in \sShieldFeasBounded^T$ is the static fairness-shield over the given time period $T$, then $\sshield\sshield\ldots$ is a periodic fairness-shield.
    \todo{define concatenation of shields}
\end{theorem}

The proof of theorem hinges on the following lemma whose proof is presented in the appendix.
\todo{Need to change the ``$a_i$'' and ``$b_i$''-s to the notation used for counters.}

\begin{lemma}\label{lem:min-frac-max}
    Let $a_1, \dots, a_m$, $b_1, \dots, b_m$ be positive real numbers. 
    Then
    \begin{equation}\label{eq:min-frac-max-lemma}
        \min_{i\in\{1\dots m\}} \frac{a_i}{b_i} \leq 
        \frac{\sum_{i=1}^m a_i}{\sum_{i=1}^m b_i} \leq 
        \max_{i\in\{1\dots m\}} \frac{a_i}{b_i}.
    \end{equation} 
\end{lemma}

==> 61_related_work_before_shortening.tex <==
% \noindent\textbf{Design-time approaches towards fair decision-making.}
Existing works on fairness address the question of how to \emph{specify}, \emph{design}, and \emph{verify} AI decision makers that are fair in their decisions.
From the specification standpoint, several criteria have been proposed to quantify fairness between groups~\cite{feldman2015certifying,hardt2016equality} and between individuals~\cite{dwork2012fairness}.
From the design standpoint, many approaches have been developed to ensure that decision-makers are fair with respect to a given fairness objective \cite{hardt2016equality,gordaliza2019obtaining,zafar2019fairness,agarwal2018reductions,wen2021algorithms}.
From the verification standpoint, several static~\cite{albarghouthi2017fairsquare,bastani2019probabilistic,sun2021probabilistic,ghosh2020justicia,meyer2021certifying,li2023certifying} and runtime~\cite{albarghouthi2019fairness,henzinger2023monitoring,henzinger2023dynamic,henzinger2023partial} approaches have been invented for verifying how fair or biased a given decision-maker is.
Our fairness shielding combines the design and verification aspects---they are \emph{verified} to be fair by \emph{design}.
Additionally, the design of our fairness shields do not require any knowledge about the underlying decision-maker, and therefore they can be used as trusted third-party intervention mechanisms to guarantee fairness of arbitrary AI-based decision makers.

Traditionally, fairness is defined using the decision-maker's output distribution.
However, it has been shown that a decision-maker that is fair according to its output distribution may exhibit biases over short horizons, which could be undesirable in many situations~\cite{pmlr-v235-alamdari24a}.
To mitigate this issue, we adopt the recently proposed bounded-horizon fairness properties~\cite{pmlr-v235-alamdari24a}, which require that decisions remain empirically fair over a given finite horizon.
To the best of our knowledge, our work is the first to provide systematic algorithmic support for guaranteeing bounded-horizon fairness properties.

We consider the setting of sequential decision making, where a fairness shield needs to make decisions without knowing the inputs from the future.
Similar problems has been extensively studied under the umbrella of optimal stopping problems~\cite{shiryaev2007optimal,bandini2018backward,ankirchner2019verification,bayraktar2020optimal,palmer2017optimal,kallblad2022dynamic}.
The focus of these works has been the analytical design of policies that are as close as possible to the hypothetical policy having the perfect foresight about the future.
Unfortunately, statistical properties like fairness remain beyond the reach of existing algorithms from the optimal stopping literature.

Our design algorithms for fairness shields are inspired by a recent work~\cite{fscd24}, which proposed sequential decision making algorithms for the general class of finite-horizon statistical properties.
They showed that the standard dynamic programming algorithm gets computationally significantly cheaper and produces the same output if the statistically indistinguishable traces are combined together.
This idea is mirrored in our design algorithm for \FinShield shields as well, where traces with the same counter values remain indistinguishable.


% On one hand they offer a minimally invasive ``course correction'' of deployed AI decision makers which is possibly designed with unknown additional objectives (like classification accuracy).
% we implement fairness by designing a symbolic decision-maker that ocassionally overrides 
% three main categories of implementation approaches were invented:
% (a) ones which \emph{pre-process} the training dataset to eliminate historical biases \cite{calders2013unbiased,kamiran2012data,zemel2013learning,gordaliza2019obtaining},
% (b) ones which design training algorithms that are robust to biases (called \emph{in-processing}) \cite{berk2017convex,zafar2017fairness,zafar2019fairness,agarwal2018reductions}, and
% (c) ones which \emph{post-process} the decision-maker's output to eliminate biases \cite{hardt2016equality}.
% Most classical implementation approaches propose \emph{design-time} techniques~\cite{calders2013unbiased,hardt2016equality,zafar2017fairness,gordaliza2019obtaining}, whereas we aim at guaranteeing fairness of already deployed decision-makers at \emph{runtime}.

% \noindent\textbf{Runtime approaches towards fair decision-making.}
% Many recent works showed how to monitor fairness of a deployed decision-maker at runtime.
% The proposed monitors are essentially online statistical estimators of biases, which would observe a long sequence of decisions made in the past, and would provide statistical estimates of how fair or biased the decision-maker has been~\cite{??}.
% % A variety of settings have been considered, namely repeated one-shot decisions, Markovian system, partially observable system states, and systems with distribution shift.
% While monitoring 


% \noindent\textbf{Bounded-horizon fairness.}

% \noindent\textbf{Online algorithms for sequential decision-making.}

% Fairness-shields are the \emph{online} counterparts of existing post-processing approaches for implementing fairness~\cite{corbett2017algorithmic}, in which predictions of AI models are post-processed to obtain 

% \todo{...}

==> 72_reproducibility_checklist.tex <==
This paper:

% \todo{Complete checklist}

\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)
\end{itemize}

Does this paper make theoretical contributions? (yes)

If yes, please complete the list below.

\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. (yes, see theorem statements)
\item All novel claims are stated formally (e.g., in theorem statements). (yes, see theorem statements)
\item Proofs of all novel claims are included. (yes, see App.~\ref{sec:detailed-proofs})
\item Proof sketches or intuitions are given for complex and/or novel results. (yes)
\item Appropriate citations to theoretical tools used are given. (yes)
\item All theoretical claims are demonstrated empirically to hold. (yes)
\item All experimental code used to eliminate or disprove claims is included. (NA)
\end{itemize}

Does this paper rely on one or more datasets? (yes)

If yes, please complete the list below.

\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets (yes)
\item All novel datasets introduced in this paper are included in a data appendix. (NA)
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (NA)
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (NA)
\end{itemize}

Does this paper include computational experiments? (yes)

If yes, please complete the list below.

\begin{itemize} 
\item Any code required for pre-processing data is included in the appendix. (yes).
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes)
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes, in the code appendix)
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes, see App.~\ref{sec:experimental_setup_appendix})
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
\item This paper states the number of algorithm runs used to compute each reported result. (yes)
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes)


\end{itemize}


==> 76_cost_alignment.tex <==
\todo{Decide which costs to present and polish this section}

In order to solve an instance of Problem~\ref{prob:bounded}, 
we need a distribution of the input space $\sgen\in \distrset(\aX)$. 
%
In the ideal case, $\sgen\in \distrset(\aG\times\BB\times\costset)$ is the exact joint distribution of group membership, agent recommendation and cost. 
However, this is unrealistic most of the time, as it assumes knowledge of the underlying distribution and the agent. 
Furthermore, the distribution of cost given by the agent may be continuous, but we assume that there is a finite set $\costset$ of costs allowed. 

In this section, we propose three ways to approximate $\sgen$, each one requiring increasing information about the underlying population distribution and the agent.
%
As a basic assumption, we assume that the distribution of the population according to their sensitive feature is known, i.e., 
we know the probability of an individual to be of group $g\in\aG$, we call it $p_g$.




\subsection{Constant approach}
The simplest approach, without any knowledge of the agent, is to assume that any recommendation is equally likely, and the cost constant.
Therefore $\costset = \{1\}$, and for all $g\in\aG$ and $r\in \BB$, 
$\sgen (g, b, 1) = p_g/2$.

\subsection{Constant 2}
If we have no knowledge of the agent, but we assume that the costs are going to be distributed over some set $\costset$, 
we can assume any recommendation and cost is equally likely. Therefore, for all $g\in\aG$, $r\in\BB$ and $c\in\costset$
\[
\sgen(g,b, c) = \frac{p_g}{2|\costset|}.
\]
This may be useful if we know beforehand the range of costs that the agent can propose. For example, if the top layer of an agent is a softmax layer, taking values between 0 and 1, one could take $\costset$ to be a discretization of the interval $[0,1/2]$ in $|\costset|$ bins.

\subsection{Hybrid}
In this case, we assume that we know the acceptance probability of the agent for both groups, 
but we do not know a distribution of costs.
Let $p_{gr}$ be the probability of making a recommendation $r\in\BB$ given that an individual is from group $g\in \aG$.
In this case, we can assume a constant cost $\costset = \{1\}$ and for each $g\in\aG$ and $r\in\BB$
\[
\theta(g, r, 1) = p_g\cdot p_{gr}
\]

\subsection{Hybrid 2}
In this case, we assume that we know the acceptance probability of the agent for both groups, 
and while we do not know the distribution of costs, 
we know they are going to be distributed over some set $\costset$.
Let $p_{gr}$ be the probability of making a recommendation $r\in\BB$ given that an individual is from group $g\in \aG$.
In this case, for all $g\in\aG$, $r\in\BB$ and $c\in\costset$
\[
\theta(g, r, c) = \frac{p_g\cdot p_{gr}}{|\costset|}.
\]

\subsection{Paired}
In this case, we assume access to the underlying population distribution and the agent. 
This is the case if we have, for example, a training fragment of the dataset $\traindata\subseteq \aF\times\aG$ and the weights of the neural network that defines the agent. 

In such cases, we can learn a histogram of costs for each group-decision pairing. To do so, first we define 
the limits of the bins
$0 = \lambda_0 \leq \lambda_1\leq \dots \leq \lambda_{n-1}  \leq \lambda_{n} = 0.5$.
Let $\Lambda_i = [\lambda_{i-1}, \lambda_i]$ for $i\in\{1,\dots,n\}$, and $c_i = (\lambda_i + \lambda_{i-1})/2$.
The cost set is $\costset = \{c_1, \dots, c_n\}$
as a discretization of the set $[0, 1/2]$ in $n$ bins.


For each $g \in \aG$ and $r \in \{0, 1\}$, 
let $N_{g, r}$ be the total number of instances in $\traindata$ of group $g$ for which the agent recommends $r$.
For each $i\in\{1,\dots,n\}$, let $N_{gri}$ be the number of instances in $\traindata$ of group $g$ in which the agent recommends $g$ and the cost of changing is inside $\Lambda_i$. Formally, this is
\[
N_{gri} = \sum_{(f',g')\in\traindata} \indicator{r = (\rho(f,g) > 0.5) \land |\rho(f,g) - 0.5|\in \Lambda_i}.
\]
Then the probability distribution is defied as
\[
    \theta(g,r,c_i) = \frac{N_{g,r,i}}{N_{g, r}}.
\]


==> 80_paper_structure_notes.tex <==
\section{Old: Paper skeleton as discussed in April}

\begin{itemize}
    \item Data-driven AI does decision making that affects our lives. Very powerful but unfair/biased.  
    \item Especially challenging in sequential decision making problems where decisions need to be make on the fly. 
    \item Decision makers need to be fair on the bounded horizon. Vaccine example.
\end{itemize}

\textbf{What was missing so far?}
    Given a learned black-box sequential decision maker, how can we be sure that any finite execution of this decision maker is fair?
    \begin{itemize}
        \item Testing: exhaustive testing too expensive
        \item Verification: Not possible due to black box (and even as white box not scalable enough)
        \item Monitoring: Just detect when execution was unfair, but too late to prevent unfair decision making.
    \end{itemize} 

\textbf{Main Idea.} 
\emph{We propose an approach to combine a data-driven descision maker with a symbolic decision maker. Advantage: Data-driven: Scalability and optimality. Symbolic decision maker: Guaranteed Fairness}

\textbf{Contribution.}
\begin{enumerate}
    \item We propose the first \emph{fair-by-construction} syntesis algorithm to construct a symbolic fair decision makers that (1) guarantee fairness on the bounded horizon and (2) minimize cost with data-driven decision makers.
    \item Propose a polynomial algorithm for the synthesis problem. The general synthesis problem of history-dependend properties is known to be PSPACE-hard. We show that for fairness properties, we have a novel polynomial algorithm. 
\end{enumerate}

%We have 4 Pages for Preliminaries + Method
\section{Preliminaries}

\section{Bounded Fairness Properties} 
Define and motivate bounded fairness properties.
Give a short example.

\section{Fairness Enforcement during Runtime}
Setting-Section.
\begin{itemize}
    \item Discuss the setting. Discuss which guarantees you provide.
    \item Discuss how to combine the data driven decision maker 
with the symbolic decision maker.
\item Continue example from before 
\end{itemize}

\section{Synthesis of Fair Symbolic Decision-Maker with Cost Minimzation}

\subsection{Static Environments}

Main Part of the Paper. Discuss algorithm and complexity.

\subsection{Dynamic Environments}

Main Part of the Paper. Discuss algorithm and complexity.


==> 83_Old_shield_definitions.tex <==
\section{Preliminary}
Let $\aX$ be some alphabet, let $\psi\colon \aX \to \{0,1\}$ we define for all $\seq{\cX}\in \aX^*$ the counting function
\begin{align*}
    \snum_{\psi}(\seq{\cX}) \coloneqq \sum_{\cX_i\in\seq{\cX}} \psi(\cX_i)
\end{align*}


\section{Shield}
We consider the following setup. 
Let $\aX\coloneqq (\aG\times \aX')$ be some feature space containing a sensitive attribute $\aG\coloneqq \{\gva,\gvb\}$ and let $\aY\coloneqq\{0,1\}$ a binary output alphabet. For any $\cX\in\aX$ we will refer to $\cX$ as member of group $\ga$, if its sensitive attribute has value $\gva$, otherwise it is considered a member of group $\gb$.

We consider a static environment $\senv\in\Delta(\aX)$ to be some distribution over the feature space $\aX$. At each point in time $t\in\NN$ the static environment generates an observation $\rX_t=(\rG_t,\rX')\sim \senv$ at random. An agent, or classifier, $\sagent\colon \aX\to \aY$ observes the randomly generated observation and produces a verdict, i.e. $\sagent(\rX_t)=\rY_t$. Hence, the interaction between the classifier and the environment generate a sequence of i.i.d. random variables $\seq{\rW}\coloneqq(\rX_t,\rY_t)_{t\in\NN}$. 



A fairness shield $\sshield\colon (\aG \times \aY )^* \times \aG \times \aY \to \aY$ considers the current sensitive attribute $\rG_t$, the current decision of the agent $\rY_t$, as well as the observed history of interactions $\seq{\rV}_{t-1}\coloneqq (\rG_i,\rZ_i)_{i\in[t-1]}$ and produces a final verdict $\rZ_t$. That is, a fairness shield has only access to the sensitive attribute. The benefit of which is that it preserves privacy and that it is agnostic to the dimension of the feature space. 

\KK{Extension?:
The properties we consider are permutation invariant fairness properties $\prop\colon (\aG \times \aY )^* \to \mathbb{R}$, i.e.\ for all $\seq{\cV}, \seq{\cV}'\in (\aG \times \aY )^*$ such that $\seq{\cV}'$ is a permutation of $\seq{\cV}$ we have that $\prop(\seq{\cV})=\prop(\seq{\cV}')$.}


We consider the commonly used fairness measure: demographic parity. That is, given a string $\seq{\cW}_{T}\in(\aX\times\aY)^*$ of length $T\in\NN$ empirical demographic parity is defined as 
\begin{align*}
    \demp(\seq{\cW}_{T})\coloneqq  \frac{\snum_{\ga\land 1}(\seq{\cW}_{T})}{\snum_{\ga}(\seq{\cW}_{T})} -\frac{\snum_{\gb\land 1}(\seq{\cW}_{T})}{\snum_{\gb}(\seq{\cW}_{T})}
\end{align*}
where $\ga(\cW)\coloneqq \indi[\cG=\ga]$ and $(\ga\land 1)(\cW)\coloneqq \indi[\cG=\gva \land \cY=1]$.


% \begin{lemma}
% Any permutation invariant fairness property $\prop$ can be expressed as a function $\prop'\colon \NN \times \NN \times \NN \to \mathbb{R}$, where for all $\seq{v}\in(\aG \times \aY )^*$ such that $|\seq{v}|=T$ we have 
% $\prop(\seq{v})=\prop'(T,\num_{\ga}(\seq{v}),\num_{1}(\seq{v}))$

% $\prop()$
% \end{lemma}
Let $T\in\NN$, let $k\in[T]$ and let $\seq{v}_k\in(\aG\times \aY)^k$


\section{Additional Results}

\begin{lemma}
    Taking the expected value of $\demp(\seq{\cW}_{T})$ recovers the usual demographic parity, as defined in the literature 
\begin{align*}
  \expe( \demp(\seq{\rW}_{T})) & = \frac{\expe(\snum_{\ga\land 1}(\seq{\rW}_{T}))}{\expe(\snum_{\ga}(\seq{\rW}_{T}))} -\frac{\expe(\snum_{\gb\land 1}(\seq{\rW}_{T}))}{\expe(\snum_{\gb}(\seq{\rW}_{T}))}  = \\
  & = \prob(\sagent(\rX) \mid \rG=\ga) -\prob(\sagent(\rX) \mid \rG=\gb)
\end{align*}
\end{lemma}
\begin{proof}
    First observe that for $\seq{\cW}_{T}\in (\aX\times \aY)^*$ such that $|\seq{\cW}_T|=T$, $\snum_{\gb}(\seq{\cW}_{T})=T-\snum_{\ga}(\seq{\cW}_{T})$.
    Next, by the tower property of conditional expectation we obtain 
    \begin{align*}
        \expe( \demp(\seq{\rW}_{T})) = \expe(\expe( \demp(\seq{\rW}_{T}) \mid \snum_{\ga}(\seq{\rW}_T)))
    \end{align*}
    Now for any fixed $k\in[T]$ we observe that 
    \begin{align*}
        \expe( \demp(\seq{\rW}_{T}) \mid \snum_{\ga}(\seq{\rW})=k)= \\
        \frac{\expe(\snum_{\ga\land 1}(\seq{\rW}_{T})\mid  \snum_{\ga}(\seq{\rW_T})=k)}{k} -\frac{\expe(\snum_{\gb\land 1}(\seq{\rW}_{T}) \mid \snum_{\ga}(\seq{\rW}_T)=k) }{T-k} 
    \end{align*}
    Moreover, observe that $\indi[\cG=\gva \land \cY=1]=\indi[\cG=\gva]\cdot \indi[ \cY=1] $. Due to permutation invariance, assume the first $k$ elements are of group $\ga$.
    \begin{align*}
        &\expe(\snum_{\ga\land 1}(\seq{\rW}_{T})\mid  \snum_{\ga}(\seq{\rW_T})=k) \\
        &=
        \sum_{i=1}^k \expe(\rY=1 \land \rG=\gva \mid \rG=\gva) +  \\
        &\, \sum_{i=k+1}^T \expe(\rY=1 \land \rG=\gva \mid \rG\neq\gva) \\
        &=
        \sum_{i=1}^k \prob(\rY=1 \land \rG=\gva \mid \rG=\gva)\\
        &=
        \sum_{i=1}^k \prob(\rY=1 \mid \rG=\gva)\cdot \prob(\rG=\gva\mid \rG=\gva)\\ 
        &= k\cdot \prob(\rY=1 \mid \rG=\gva)
    \end{align*}
    Therefore, 
    \begin{align*}
  \expe( \demp(\seq{\rW}_{T})) &=  \expe(\prob(\sagent(\rX) \mid \rG=\ga) -\prob(\sagent(\rX) \mid \rG=\gb)) \\
  &= \prob(\sagent(\rX) \mid \rG=\ga) -\prob(\sagent(\rX) \mid \rG=\gb)
\end{align*}
\end{proof}


\section{Old 2}




 




% \begin{remark}
%     We can generalize the classifier to be a history dependent agent 
%     $\sagent\colon (\aX\times \aY\times \aY)^* \times \aX \to \aY$.
%     Under this condition the soundness result still holds, however, the optimality guarantee is lost. By contrast, if the agent remains agnostic to the decisions of the shield, the optimality result holds. 
% \end{remark}






\section{Old}
Next we will discuss the enforcement problem in a simplified setting. 
Namely, we will look a a scenario where the environment is independent of the actions of the agent and the shield, and the agent is agnostic to the interventions of the shield.

\begin{example}
    As common in machine learning we assume a static distribution $\distr$ over $\aX$. Moreover, let $\mathcal{N}:\aX\to\{0,1\}$ neural decision maker trained w.r.t.\ $\mathcal{D}$. During deployment we sequentially observe $T\in\NN$ independent samples $\rX_1, \dots, \rX_T$ from $\mathcal{D}$, i.e.\ the environment does not change based on the decision of the neural network or any potential shield. 
    Moreover, $\mathcal{N}$ only takes values of $\aX$ as input, thus it is agnostic of the decisions of any potential shield. 
\end{example}


Let $\aX\coloneqq\aX'\times\aG$ be alphabet of the environment, where $\aG\coloneqq\{\ga,\gb\}$ is the set of sensitive attributes and $\aX'$ is the remaining feature space. Moreover, let $\aY=\aY=\{0,1\}$ be the output alphabet of the agent and the shield respectively. 
% Let $\aH\coloneqq (\aX\times  \aS)$ and $\aF\coloneqq (\aX\times \aA \times \aS)$, we call $\seq{\cH} \in \aH^*$ a history and $\seq{\cF} \in \aF^*$ a full history.
We define the environment to be $\senv\colon (\aX\times \aY)^*\to \Delta(\aX)$, agent to be $\sagent\colon (\aX \times \aY\times \aY)^*\times  \aX \to  \aY$, and the shield to be $\sshield\colon (\aX \times \aY\times \aY)^* \times\aX \times \aY \to  \aY$. Next we define the marginal environment, i.e.\ for $\cG\in\aG$ and $\seq{\cV} \in(\aX\times \aY)^*$ as 
\begin{align*}
    \senvg(\seq{\cV})(\cG) \coloneqq \int_{\aX'} \senvg(\seq{\cV})(\cX',\cG) \; \mathrm{d}\cX'
\end{align*}
Since the $|\aG|=2$ the marginal environment is a Bernoulli distribution with parameter $\sgp(\seq{\cV})\coloneqq \senvg(\seq{\cV})(\ga)$.
An environment is $\lip$-group-Lipschitz, if there exists an $\lip\geq0$ such that for all $\seq{\cV}, \seq{\cV}',\seq{\cV}''\in (\aX\times \aY)^*$ such that $k=|\seq{\cV}'|=|\seq{\cV}''|$ we have 
\begin{align*}
    |\sgp(\seq{\cV}\cdot \seq{\cV}') - \sgp(\seq{\cV}\cdot \seq{\cV}'')| \leq t\cdot \lip
\end{align*}


We are interested in developing a shield for ensuring demographic parity.
We define demographic parity as follows. Let $\seq{\cV} \in  (\aX\times \aY)^*$ with $T=|\seq{\cV}|$. For $\cG\in\aG$, let $\snum_{\cG}(\seq{\cV})\coloneqq \sum_{i=1}^T \indi\{\cX_i=\cG\}$ and $\snum_{1\mid\cG}(\seq{\cV})\coloneqq \sum_{i=1}^T \cZ_i\cdot \indi\{\cX_i=\cG\}$
\begin{align*}
    \varphi(\seq{\cV}_T)\coloneqq \frac{\snum_{1\mid\ga}}{\snum_{\ga}} - \frac{\snum_{1\mid\gb}}{\snum_{\gb}} 
\end{align*}



Let $T\in\NN$, let $k\in[T]$, let $\delta\in(0,1)$, let $\varepsilon>0$, we want to find a shield $\sshield$ such that for all agents $\sagent$ and all $\lip$-group-Lipschitz environments the condition
\begin{align*}
    \prob_{\senv, \sagent, \sshield}\left( |\varphi(\seq{\rV}_T) |\leq \varepsilon \right) \geq \delta
\end{align*}



\begin{problem}\label{prob:general}
	Let $T \in \mathbb{N}$ be the given horizon length (i.e., the last stage index), $\env$ be the given stochastic generator, $\pay$ be the given reward function, and  $\con$ be the given cost function.
    % Let $\Sysfeas^\env\subseteq \Sys$ be the set of feasible transducers fulfilling the cost constraint in the presence of $\env$, i.e.,
    % \begin{equation}\label{eq:general:constraint}
    %     \Sysfeas^\env \coloneqq \set{\sys\in\Sys \mid \forall \seq{\cio}_T\in \dom(\prob_{\env,\sys})\;.\;\con(\seq{\cio}_T) = 1}.
    % \end{equation}
	Compute the \emph{optimal} transducer $\sys^*$ that is feasible and is reward-optimal, i.e.,
    \begin{equation}
        \label{eq:prob:general:obj}
        \sys^* = \arg \max_{\sys\in \Sysfeas^\env}\, \expe_{\env,\sys}\left[  \pay\right].
    \end{equation}
	We will call the tuple $\tup{\AI,\AO,\env,\pay,\con,T}$ a \emph{problem instance}.
\end{problem}

==> 84_synthesis_usingMDP.tex <==

We first consider the bounded-horizon synthesis problem, formulated in Prob.~\ref{prob:bounded}.
In theory, the optimization problem can be solved by constructing the underlying Markov decision process (MDP) that models the turn-based interactions between the agent and the shield, where each state of the MDP stores the input-output history, the probabilistic transitions represent the probabilistic generation of inputs from $\aX$, and the non-deterministic actions represent the shield's outputs from $\aY$.
Since the horizon is finite, therefore the state space of the MDP is also finite, and therefore standard value-iteration algorithms could be used to compute optimal shield policy.
Unfortunately, this approach would not scale for larger horizons, since the size of the MDP would grow exponentially with respect to the horizon $T$.
We call this the \emph{exact} approach, and the respective MDP the \emph{exact} MDP.

To alleviate this blow-up, we use the statistical abstraction-based approach proposed by Cano et al.~\cite{?} for similar class of sequential decision-making problems under probabilistic uncertainties.
The key observation is that the shield's output, after seeing the current input, would not require the full input-output history, but will only depend on the \emph{statistics} about the history that is relevant to DP (number of accepted and appeared individuals from each group). 
Therefore, all states containing the same statistical information can be clustered together without sacrificing the shield's optimal policy.
The resulting MDP will have a significantly smaller state space, and will be called the \emph{abstract} MDP.
It turns out that the state space of the abstract MDP would grow only polynomially with respect to $T$.
We summarize the abstraction and policy synthesis approach below; details can be found in the paper by Cano et al.~\cite{?}.


In our case, the relevant statistics about the past are encoded using four counters whose values are denoted using the variables $n_a,n_{a1},n_b,n_{b1}\in\NN$, where for each $g\in \set{a,b}$, $n_g$ represents the number of individuals appeared from group $g$ and $n_{g1}$ represents the number of individuals accepted from group $g$.
Observe that each of the four counters take values within the bounded range $[0;T]$, where $T$ is the time horizon.
For a given $(n_a,n_{a1},n_b,n_{b1})\in [0;T]^4$, with a slight abuse of notation, we will use the notation
\begin{align*}
    \DP(n_a,n_{a1},n_b,n_{b1}) = \left| \frac{n_{a1}}{n_a} - \frac{n_{b1}}{n_b} \right|,
\end{align*}
assuming $n_a,n_b>0$.
When $n_a$ or $n_b$ is zero, we say $\DP(n_a,n_{a1},n_b,n_{b1})$ is undefined.

\begin{definition}\label{def:abstract mdp}
    The abstract MDP is the tuple $\tup{\Vr, \Vc, \vinit, \Probr,\Tran,\costmdp}$ where
    \begin{itemize}
        \item $\Vr = \set{(n_a,n_{a1},n_b,n_{b1})\in [0;T]^4\mid n_a+n_b\leq T \land n_{a1}\leq n_a\land n_{b1}\leq n_b}$ is the set of \emph{environment states},
        \item $\Vc = \Vr\times \aX$ is the set of \emph{decision states},
        \item $\vinit$ is the \emph{initial state} that belongs to $\Vr$ and is fixed to $(0,0,0,0)$,
        \item $\Probr\colon \Vr\times\Vc\to [0,1]$ is the probability kernel for the \emph{environment transitions} such that $\Probr(q,(q,\cX)) = P_\sagent(\cX)$,
        \item $\Tran\subseteq \Vc\times\aY\times \Vr$ is the transition relation from the decision states such that for every $(n_a,n_{a1},n_b,n_{b1},\cX = (g,\cdot,\cdot))$ with $n_a+n_b\neq T$ and for every $\cY\in\aY$, we have $((n_a,n_{a1},n_b,n_{b1},\cX),\cY,(n_a',n_{a1}',n_b',n_{b1}'))\in \Tran$ iff:
        \begin{itemize}
            \item If $g=a$ (i.e., the ``input individual'' is from group $a$), then $n_a'=n_a+1$, and, moreover, if $y=1$ (i.e., the individual is accepted) then $n_{a1}' = n_a+1$ and else $n_{a1}'=n_{a1}$.
            The variables $n_b',n_{b1}'$ remain the same as $n_b,n_b$, respectively.
            \item The case of $g=b$ is defined analogously.
        \end{itemize}
        \item $\costmdp\colon T\to \RR_{\geq 0}$ is the cost function such that for every transition $\mathit{tr}=((\cdot,\cdot,\cdot,\cdot,\cX=(\cdot,r,c)),\cY,(n_a',n_{a1}',n_b',n_{b1}'))\in \Tran$,
        \begin{itemize}
            \item If $n_a'+n_b'<T$ (the horizon has not been reached yet), then $C(\mathit{tr})=c$ if $\cY\neq r$ (the shield deviates from the agent's recommendation), and $C(\mathit{tr})=0$ otherwise.
            \item If $n_a'+n_b'=T$ (the horizon has been reached), then $C(\mathit{tr})=\infty$ if $\DP(n_a',n_{a1}',n_b',n_{b1}') > \kappa$ (empirical DP is violated), and $C(\mathit{tr})=0$ otherwise.
        \end{itemize}
    \end{itemize}
\end{definition}

Every environment state $(n_a,n_{a1},n_b,n_{b1})\in\Vr$ of the abstract MDP for which $n_a+n_b=T$ is a sink state, i.e., without any outgoing transition.
It can be easily verified that every path of the abstract MDP that starts at the initial state reaches the sink state in exactly $2T$ steps.

The semantics of the abstract MDP is as usual interpreted over the probability distribution over the paths (sequence of states) for a given \emph{policy} of the form $(\Vc\times \Vr)^{< T}\times\Vc \to \aY$; the semantics of MDP can be found in standard textbooks~\cite{?}.
\todo{Explain a little bit about total expected cost.}
The bounded-horizon fairness-shield synthesis problem reduces to finding the optimal policy in the abstract MDP that minimizes total expected cost.

% --------- Abstract MDP defined in the text -----------------
% The abstract MDP contains two types of states: the \emph{environment states}, which belong to $[1;T]^4$ and contain the input-output statistics of the past, and the \emph{decision states}, which belong to $[1;T]^4\times \aX$ and contain both the statistics and the current input.
% Therefore, the size of the state space of the abstract MDP is $\mathcal{O}(T^4\cdot |\aX|)$.
% \footnote{In reality, the size of the state space will be much smaller because the set of statistics will contain only those counter values $(n_a, n_{a1}, n_b, n_{b1})$ for which $n_a+n_b\leq T$.}
% Every environment state $(n_a,n_{a1},n_b,n_{b1})$ transitions to the decision state $(n_a,n_{a1},n_b,n_{b1},\cX)$ with probability $P_\sagent(\cX)$ in the next step.
% On the other hand, at every decision state $(n_a,n_{a1},n_b,n_{b1},\cX = (g,f,r,c))$, the shield needs to choose an output $\cY\in\aY$, based on which the abstract MDP transitions to the new environment state $(n_a',n_{a1}',n_b',n_{b1}')$ defined as follows:
% Suppose $g=a$ (i.e., the ``input individual'' is from group $a$).
% Then $n_a'=n_a+1$, and, moreover, if $y=1$ (i.e., the individual is accepted) then $n_{a1}' = n_a+1$ and else $n_{a1}'=n_{a1}$.
% The variables $n_b',n_{b1}'$ remain the same as $n_b,n_b$, respectively.
% The case of $g=b$ is defined analogously.
% The abstract MDP always starts at the initial environment state $(0,0,0,0)$, and stops at the sink environment states from the set $\set{(n_a,n_{a1},n_b,n_{b1})\mid n_a+n_b=T}$.
% It can be verified that every path of the abstract MDP that starts at the initial state reaches the sink state in exactly $2T$ steps.
% ------------------------------------------

% ------------- cost function defined in text -----------------
% Finally, we can assign costs to each transition of the abstract MDP in a way that every policy which minimizes the total expected cost, upon reaching a sink, is a cost-optimal shield over the horizon $T$ in Prob.~\ref{prob:bounded}.
% The costs are defined as follows.
% Every outgoing transition from every environment state has zero cost.
% Suppose $\mathit{tr}$ is a transition originating from the decision state $(n_a,n_{a1},n_b,n_{b1},\cX = (g,f,r,c))$, triggered by the shield's output $\cY$, and ending at the new environment state $(n_a',n_{a1}',n_b',n_{b1}')$.
% If $n_a'+n_b'<T$ (the horizon has not been reached yet), then the cost of the transition $\mathit{tr}$ is $c$ if $\cY\neq r$ (the shield deviates from the agent's recommendation), and is zero otherwise.
% If $n_a'+n_b'=T$ (the horizon has been reached), then the cost of $\mathit{tr}$ is $\infty$ if $\DP_\kappa(n_a',n_{a1}',n_b',n_{b1}') = 0$ (empirical DP is violated), and is zero otherwise.
% ---------------------------------------------------------


The optimal policy synthesis problem on the abstract MDP can be solved using the well-known value iteration approach that can be shown to run in $\mathcal{O}(|\Vc|)$-steps.
The following theorem follows.

\begin{theorem}\label{thm:bounded-horizon shield synthesis}
    The bounded-horizon shield-synthesis problem can be solved in $\mathcal{O}(T^4\cdot |\aX|)$-time.
\end{theorem}

In practice, the abstract MDP is built only implicitly during the value iteration algorithm; details were presented in~\cite{fscd24}.



% The dynamic programming will simultaneously compute two separate sets of value functions
% denoted as $\set{v_t}_{t\in [1;T]}$ and $\set{w_t}_{t\in[1;T]}$.
% Each function $v_t$ is of the form $(n_a,n_{a1},n_b,n_{b1})\mapsto \RR$, which represents the additional expected cost that needs to be incurred given that the current time step is $t$ and the current counter values are $n_a,n_{a1},n_b,n_{b1}$.
% On the other hand, each function $w_t$ is of the form $((n_a,n_{a1},n_b,n_{b1}),(g,f,r,c))\to \RR$, which represents the additional expected cost that needs to be incurred given that the current time step is $t$, the current counter values are $n_a,n_{a1},n_b,n_{b1}$, and the current input is $(g,f, r,c)$.
% From the definition of expected values, it follows that for every $t\in [1;T-1]$, 
% \begin{align}
%     v_t(N) = \sum_{x\in \aX} w_t(N, x)\cdot P_\sagent(x).
% \end{align}
% On the other hand, $w_t(N,x)$ 

% every counter valuation $N = (n_a,n_{a1},n_b,n_{b1})\in [1;T]^4$ to a positive real number as follows.
% % \begin{figure*}
% \begin{align*}
%     &\forall t\in [1;T-1]\;:\;\\ &\quad v_t(N) = \sum_{x\in \aX} w_t(N, x)\cdot P_\sagent(x),\\
%     &\quad w_t\left(N, x = (g, f, r, c)\right) = \\
%     &\qquad\min\left\lbrace 
%         \begin{matrix}
%             v_{t+1}(n_a+1,n_{a1}+1,n_b,n_{b1}) + c\cdot \indicator{r=0}\\
%             v_{t+1}(n_a+1,n_{a1},n_b,n_{b1})+ c\cdot \indicator{r=1}
%         \end{matrix}
%     \right\rbrace,\\
%     &t=T\;:\;\\
%     &\quad v_{t}(N) =
%         \begin{cases}
%             \infty & \text{if } \DP_\kappa(\sem{N}) =0,\\
%             0   &   \text{otherwise.}
%         \end{cases}
% \end{align*}
% % \end{figure*}

\todo{
\begin{itemize}
    \item  State the soundness theorem of the value iteration, and state how the shield policy can be extracted from the value iteration steps.
    \item Optimization: We can consider an abstraction over $\aF$ so that the sum in the definition of $v_t$ contains fewer terms. For this, we will need to redefine $P_\sagent$ in a way that it does not depend on all the features in $\aF$.
    \item A subsection on the cost output by the agent: Two alternatives: constant cost, suitable for when we don't know anything about the classifier, and a real valued variable cost, suitable when the classifier outputs some real number between $0$ and $1$, and then the classification decision is done by using a threshold value (the cost will depend on the distance from the threshold).
\end{itemize}

}

==> 85_compositional_full_discussion.tex <==
\section{An Attempt towards a Compositional Approach}

Let us try to answer the following question: If we have been fair (as per demographic parity) in the first "time window," what should the enforcer do in the following time windows so that we are fair in the combined window? 
Let us formalize this first.
Let $i$ be the index of the time window, and $t_i = (a_i,b_i,p_i,q_i)$ denote the number of individuals who were accepted from group A, total number of individuals seen from group A, number of individuals who were accepted from group B, and the total number of individuals seen from group B, in the time window $i$.

The demographic parity after $m$ windows is:
\begin{equation}
    DP(t_1,\dots, t_m) = \left| 
    \frac{\sum_i a_i}{\sum_i b_i} -
    \frac{\sum_i p_i}{\sum_i q_i} 
    \right|.
\end{equation}

We want to investigate under which conditions of $\{t_i\}_{i:1\dots m}$ can we guarantee that $DP(t_1,\dots,t_m)<\kappa$, for a given $\kappa$.

The first natural solution is to move the target on DP to take into account previously seen values.

\begin{definition}[Buffered Demographic Parity]
    Let $\bar t = (\bar a, \bar b, \bar p, \bar q)$ represent the accumulated number of individuals accepted from group A, seen from Group A, accepted from group B and seen from group B, respectively. For a new tuple $t = (a,b,p,q)$, the \emph{buffered demographic parity} is:
    \begin{equation}
        BDP_{\bar a, \bar b, \bar p, \bar q}(a,b,p,q) = 
        \left| 
        \frac{\bar a + a}{\bar b + b} -
        \frac{\bar p + p}{\bar q + q} 
        \right|.
    \end{equation}
\end{definition}


\begin{proposition}\label{prop:bdp}
    Let $\{t_i\}_{i:1\dots m}$ be tuples, and let 
    $\bar t_i = \sum_{j = 1}^{i-1} t_j$. 
    If $t_{i}$ is chosen such that $BDP_{\bar t_i}(t_i) < \kappa$ for all $i$, 
    then $DP(t_1, \dots, t_m) < \kappa$.
\end{proposition}

This proposition is true by construction, and provides a natural incremental shielding approach: at the end of every time window, a new shield has to be synthesized with a specification in terms of buffered DP instead of DP. 

The drawback of this approach is that it requires the user to synthesize a shield anew for every time window. 
If we would have a condition on the DP of each tuple, instead of BDP, 
we could use the same shield at every time window. 

The first intuition is that if $DP(t_1) < \kappa$ and $DP(t_2) < \kappa$,
then it should be that $DP(t_1,t_2) < \zeta \kappa$, for some small constant $\zeta$.
The following result proves that such $\zeta$ cannot be independent of $\kappa$ and the size of the window.

\begin{theorem}\label{thm:K(N-K)}
    For every $\varepsilon > 0$, 
    there exists $N>0$, and natural number tuples $(a_i, b_i, p_i, q_i)$ for $i\in \{1,2\}$ such that:
    \begin{enumerate}
        \item $b_i + q_i = N$ for $i\in \{1, 2\}$, 
        \item $DP(a_i, b_i, p_i, q_i) < \varepsilon$ for $i\in \{1, 2\}$, and
        \item $DP(a_1 + a_2, b_1 +b_2, 
        p_1 + p_2, q_1 + q_2 > 1 - \varepsilon$.
    \end{enumerate}
\end{theorem}

\begin{proof} (Sketch only)

    This proof is done by constructing a family of counterexamples, parametrized by $N > 0$ and $ 0 < K < N/2$. 
    For a pair $(N,K)$ consider the tuples $t_1 = (1, K, 1, N-K)$ and $t_2 = (N-K-1, N-K, K-1, K)$. 
    In the window $t_1$, exactly one element of each group was accepted, while in the window $t_2$, all but one element of each group were accepted. 
    Let's compute demographic parities for this example.

    \begin{equation} \label{eq:dp1}
        DP^1_{N,K} = \left|
        \frac{1}{K} - \frac{1}{N-K}\right| = \frac{N-2K}{(N-K)K}
    \end{equation}

    \begin{equation}\label{eq:dp2}
        DP^2_{N,K} = \left|
        \frac{N-K-1}{N-K} - \frac{K-1}{K}
        \right| = 
        \frac{N-2K}{(N-K)K}
    \end{equation}

    \begin{equation}\label{eq:dp1+2}
        DP^{1+2}_{N,K} = \left|
        \frac{N-K}{N} - \frac{K}{N}
        \right| = 
        \frac{N-2K}{N}
    \end{equation}

    The key observation is that, once fixed $K$, the limit when $N\to \infty$ of Eq.~\ref{eq:dp1} and Eq.~\ref{eq:dp2} is $1/K$, but the limit when $N\to\infty$ of Eq.~\ref{eq:dp1+2} is 1.
    Therefore, for every $\varepsilon$, we can find $K$ large enough such that $1/K < \varepsilon/2$, 
    and then find $N$ large enough such that the corresponding $DP$ values are close enough to the limit.
\end{proof}    


\begin{theorem}
    Let $n$ be a window size. There exist two tuples $t_1, t_2$
    with $DP(t_i) = 0$ 
    such that $DP(t_1, t_2) = \frac{n-2}{n}$.
\end{theorem}

\begin{proof}

    Consider the two tuples $t_1 = (0, 1, 0, n-1)$ and $t_2 = (n-1, n-1, 1, 1)$. 
    Clearly $DP(t_i) = 0$.

    \begin{equation}
        DP(t_1, t_2) = \left| 
        \frac{n-1}{n} - \frac{1}{n}
        \right| = \frac{n-2}{n}
    \end{equation}
    
\end{proof}

An approach that does work is to bound not only the DP, but also the acceptance rates of each of the groups.
This approach has nice compositional properties, as illustrated by the following result:

\begin{theorem}\label{thm:beta-alpha}
    Let $\alpha\leq \beta$ be two constant numbers between 0 and 1.
    Let $\{t_i\}_{i:1\dots m}$ be tuples such that 
    $\alpha \leq a_i/b_i \leq \beta$ and 
    $\alpha \leq p_i/q_i \leq \beta$ for all $i$. 
    Then 
    $DP(t_1,\dots, t_m) < \beta - \alpha$.
\end{theorem}

To prove Thm.~\ref{thm:beta-alpha}, we need the following auxiliary result.

\begin{lemma}\label{lem:min-frac-max}
    Let $a_1, \dots, a_m$, $b_1, \dots, b_m$ be positive real numbers. 
    Then
    \begin{equation}\label{eq:min-frac-max-lemma}
        \min_{i\in\{1\dots m\}} \frac{a_i}{b_i} \leq 
        \frac{\sum_{i=1}^m a_i}{\sum_{i=1}^m b_i} \leq 
        \max_{i\in\{1\dots m\}} \frac{a_i}{b_i}.
    \end{equation} 
\end{lemma}
\begin{proof}
    We prove this result by induction on $m$. The base case for $m=1$ is trivial. 
    For a general $m$, we will use the following inequality:
    for positive numbers $w, x, y, z$, if $w/x < y/z$, then
    $\frac{w}{x} \leq \frac{w+y}{x + z} \leq \frac{y}{z}$. 
    This is a well-known result, and we can restate it as:
    \begin{equation} \label{eq:min-frac-max1}
        \min\left(
        \frac{w}{x}, \frac{y}{z} 
        \right)
        \leq \frac{w + y}{x + z} 
        \leq 
        \max\left(
        \frac{w}{x}, \frac{y}{z} 
        \right)
    \end{equation}
    We will apply inequality~\ref{eq:min-frac-max1} with
    $w = \sum_{i=1}^{m-1} a_i$, 
    $x = \sum_{i=1}^{m-1} b_i$,
    $y = a_m$, and $z = b_m$, 
    to obtain:
    \begin{equation*}
        \frac{\sum_{i=1}^m a_i}{\sum_{i=1}^m b_i} \leq
        \max\left(
        \frac{\sum_{i=1}^{m-1} a_i}{\sum_{i=1}^{m-1} b_i}, 
        \frac{a_m}{b_m}
        \right).
    \end{equation*}
    Applying the induction hypothesis we have that 
    \begin{equation}
        \frac{\sum_{i=1}^{m-1} a_i}{\sum_{i=1}^{m-1} b_i} \leq 
        \max_{i\in \{1\dots m-1\}} \frac{a_i}{b_i},
    \end{equation}
    and therefore:
    \begin{equation*}
        \frac{\sum_{i=1}^m a_i}{\sum_{i=1}^m b_i} \leq
        \max\left(
        \max_{i\in \{1\dots m-1\}} \frac{a_i}{b_i}, 
        \frac{a_m}{b_m}
        \right) = \max_{i\in \{1\dots m\}} \frac{a_i}{b_i}.
    \end{equation*}
    This proves the right-side inequality of Eq.~\ref{eq:min-frac-max-lemma}. 
    The left-side is analogous.
\end{proof}

\begin{proof}[Proof (Of Theorem~\ref{thm:beta-alpha})]
    For one tuple $t = (a,b,p,q)$, we have that $a/b \leq \beta$ 
    and $p/q \geq \alpha$, therefore $-p/q < -\alpha$. 
    Putting this together we have
    \begin{equation} \label{eq:beta-alpha}
        \frac ab - \frac pq \leq \beta - \alpha.
    \end{equation}
    On the other hand, we have that $a/b \geq \alpha$
    and $p/q \leq \beta$, therefore $-p/q \geq -\beta$. 
    Putting this together we get
    \begin{equation} \label{eq:alpha-beta}
        \frac ab - \frac pq \geq \alpha - \beta = -(\beta - \alpha).
    \end{equation}
    With equations~\ref{eq:beta-alpha} and~\ref{eq:alpha-beta} together, 
    we get $DP(a,b,p,q) \leq \beta - \alpha$.

    Using Lemma~\ref{lem:min-frac-max}, we have that 
    \begin{equation*}
       \alpha \leq \min_i \frac{a_i}{b_i} \leq 
        \frac{\sum_i a_i}{\sum_i b_i} \leq 
        \max_i \frac{a_i}{b_i} \leq \beta, \quad \mbox{and}
    \end{equation*}
    %
    \begin{equation*}
        \alpha \leq \min_i \frac{p_i}{q_i} \leq 
        \frac{\sum_i p_i}{\sum_i q_i} \leq 
        \max_i \frac{p_i}{q_i} \leq \beta.
    \end{equation*}
    Therefore, we can apply Eqs.~\ref{eq:beta-alpha} and~\ref{eq:alpha-beta} to the tuple 
    $\bar t~=~\left(
    \sum_{i=1}^m a_i, \sum_{i=1}^m b_i, 
    \sum_{i=1}^m p_i, \sum_{i=1}^m q_i
    \right)$
    to finish the proof.    
\end{proof}


If we try to build shields using Th.~\ref{thm:beta-alpha}, 
we soon arrive to the issue that it may not be possible to 
ensure an acceptance rate between a given interval $(\alpha, \beta)$. 
Consider, for example, $\alpha = 0.2$, $\beta = 0.3$. 
If in a given run, only 3 elements of group A appear, 
the acceptance rates can only be $0$, $1/3$, $1/2$, $2/3$, and $1$, 
all outside the target interval. 

To ensure that enough candidates appear of a given group, we need to solve the following problem.

\begin{problem}\label{prob:alpha-xn-beta}
    Given $0 \leq alpha < \beta \leq 1$, find $N$ such that for all $n\geq N$, there exists $x_n\in\mathbb N$ such that 
    \begin{equation}
        \alpha \leq \frac{x_n}{n} \leq \beta, \quad \mbox{and} 
        \quad x_{n+1} - x_n \in \{0,1\}.
    \end{equation}
\end{problem}

Given $\alpha$, and $\beta$, if there are at least $N$ incoming candidates of a given group, the shield can accept exactly $x_n$ to ensure the condition on bounded acceptance rates is met. 

\begin{lemma}
    A solution to Problem~\ref{prob:alpha-xn-beta} is $N = \left\lceil \frac{1}{\beta-\alpha}\right\rceil$.
\end{lemma}

\begin{proof}
    The condition in Problem~\ref{prob:alpha-xn-beta} can be reformulated as $\alpha n \leq x_n \leq \beta n$,
    and since $x_n$ needs to be an integer, 
    we can tighten it to 
    \begin{equation}\label{eqn:local1}
        \left\lceil \alpha n \right\rceil \leq x_n \leq 
        \left\lfloor \beta n \right\rfloor.
    \end{equation}
    One option is to try $x_n = \left\lceil \alpha n \right\rceil$.
    We have to prove that this choice satisfies two conditions: 
    (i) $x_{n+1} - x_n \in \{0,1\}$, and
    (ii) Equation~\ref{eqn:local1}.

    \begin{enumerate}
        \item[(i)] $x_{n+1} - x_n = \lceil \alpha(n+1)\rceil - \lceil \alpha n\rceil$. 
        For any number $x$, it is known that $x \leq \lceil x\rceil < 1$. Applying this inequality twice, we get 
        $\lceil \alpha(n+1)\rceil - \lceil \alpha n\rceil < \alpha (n+1) - \lceil\alpha n\rceil \leq \alpha(n+1)-\alpha n = 1+\alpha < 2$. 
        Since $\lceil \alpha(n+1)\rceil - \lceil \alpha n\rceil$ is an integer strictly smaller than 2, it is smaller or equal than 1. It is also clearly non-negative.

        \item[(ii)]
        By construction, $\alpha n \leq \lceil\alpha n\rceil$. 
        Now we have to see that $\lceil\alpha n\rceil \leq \beta n$. 
        If $\lceil\alpha n\rceil = \alpha n$, 
        then for any $n\geq 1$, $x_n \leq \beta n$ on account of $\alpha < \beta$. 
        If $\lceil\alpha n\rceil = \alpha n +1$, 
        we need $\alpha n + 1 \leq \beta n$, 
        which is equivalent to $n \geq \frac{1}{\beta - \alpha}$. 
        Since $n$ needs to be an integer, selecting $N = \left\lceil \frac{1}{\beta-\alpha}\right\rceil$ ensures this condition is satisfied. 
    \end{enumerate}
\end{proof}

While it is possible to find tighter conditions for concrete values of $\alpha$ and $\beta$, the construction in the proof illustrates that this is the best bound for general values of $\alpha$ and $\beta$. 
\FC{I'm not sure about this last sentence. }

Note that the feasiblity of this condition depends on the values of $\alpha$ and $\beta$ to enforce, as well as the incoming probability distribution. 
In its most simplified form, if we just care about the group membership of any incoming candidate, the distribution of incoming candidates follows a Bernoulli distribution $B(p)$, where $p$ is the probability to receive a candidate of group A. 
After a time horizon $T$, the number of incoming candidates of group A follows a binomial distribution $Bin(T, p)$, and the probability to see at least $N$ candidates of each group is the probability of the binomial being between $N$ and $T-N$, which is 
\[
\sum_{k=N}^{T-N}\binom{T}{k}p^k(1-p)^{T-k}.
\]
In practice, this corresponds to the probability that our shield will encounter a trace where demographic parity with the given bound on acceptance rates can be enforced. 
It is up to the user to evaluate whether this guarantee is enough for a given application.


% \vspace{1cm}
% \subsection{Kept for safekeeping}
% \FC{I keep this here before deleting, but to my understanding, the results in the following theorem are subsumed under Prop.~\ref{prop:bdp} and Theorem~\ref{thm:beta-alpha}}.

% Let us consider only a one-sided demographic parity, where ultimately we want to achieve
% \begin{align}\label{eq:fairness in two windows}
% 0<\frac{a_1+a_2}{b_1+b_2}-\frac{p_1+p_2}{q_1+q_2} < K,
% \end{align}
% for a given positive constant $K$.
% Suppose at the end of the first time-window, the enforcer achieved
% \begin{align}\label{eq:fairness in the first window}
% 0<\frac{a_1}{b_1}-\frac{p_1}{q_1} < K.
% \end{align}
% What should the enforcer do in the second window to achieve \eqref{eq:fairness in two windows}?
% Here is an idea.

% \begin{theorem}
% If in the second time window (of arbitrary length), the enforcer guarantees both of the following,
% \begin{align}
%     &\frac{a_2}{b_2}>\frac{a_1}{b_1} > \frac{p_2}{q_2} > \frac{p_1}{q_1}\label{eq:thm:a}\\
%     &\frac{a_2}{b_2} - \frac{p_1}{q_1} < K.\label{eq:thm:b}
% \end{align}
% then \eqref{eq:fairness in two windows} is fulfilled.
% \end{theorem}

% \begin{proof}
%     First, observe that, for every real $w,x,y,z$, if $\frac{w}{x}<\frac{y}{z}$, then
%     \[
%     \frac{w}{x} < \frac{w+y}{x+z} < \frac{y}{z}.
%     \]
%     Let us prove this.
%     For the first inequality:
%     \begin{align*}
%         &\frac{w}{x} < \frac{y}{z}\\
%         \implies& wz < yx\\
%         \implies& wz + wx < yx + wx\\
%         \implies& w(z+x) < x(y+w)\\
%         \implies& \frac{w}{x} < \frac{w+y}{x+z}.
%     \end{align*}
%     For the second inequality:
%     \begin{align*}
%         &\frac{w}{x} < \frac{y}{z}\\
%         \implies& wz < yx\\
%         \implies& wz + yz < yx + yz\\
%         \implies& z(w+y) < y(x+z)\\
%         \implies& \frac{w+y}{x+z} < \frac{y}{z}.
%     \end{align*}
%     Therefore, from the first inequality in \eqref{eq:thm:a} it follows that
%     \begin{align}\label{eq:c}
%             \frac{a_2}{b_2} > \frac{a_1+a_2}{b_1+b_2} > \frac{a_1}{b_1},
%     \end{align}
%     and from the second inequality in \eqref{eq:thm:a}
%     \begin{align}\label{eq:d}
%             \frac{p_2}{q_2} > \frac{p_1+q_2}{p_1+q_2} > \frac{p_1}{q_1}.
%     \end{align}
%     From \eqref{eq:thm:a}, \eqref{eq:c}, and \eqref{eq:d}, we obtain:
%     \begin{align*}
%         \frac{a_2}{b_2}> \frac{a_1+a_2}{b_1+b_2} > \frac{p_1+q_2}{p_1+q_2} > \frac{p_1}{q_1}.
%     \end{align*}
%     Finally, the claim of the theorem follows by using \eqref{eq:thm:b}.
% \end{proof}

% After the second time window, we can treat the combined first and second windows as the ``new first window'' and keep repeating the process.



==> 86_empirical_DP_estimator.tex <==
Let $\p$ be the probability of observing a member of group $a$, let $p_{1|g}$ be the actual probability of a member of group $g\in\aG$ of being accepted.
Moreover, given a trace $\trace$ let $n_g$ and $n_{1\mid g}$ be the number of observed and accepted members of group  $g\in\aG$ respectively. The corresponding random quantities are $N_g$ and $N_{1\mid g}$

The empirical demographic parity %, as defined in Eq.~\ref{eq:DP-definition}
is an estimator of the real demographic parity, and as such, it is expected to have errors. From a statistical perspective, it is easier to analyse what we will call \emph{signed} demographic parity, which corresponds to $\sdp = \pa - \pb$.
We define the empirical \emph{signed} demographic parity for every $T\in \NN$, $\cn, \cna, \cnb \in [T]$ as 
\begin{align*}
    \sdp(\cn, \cna, \cnb) \coloneqq \begin{cases}
        \frac{\cna}{\cn}-\frac{\cnb}{T-\cn}   & \quad 0<\cn<T \\
        0 & \quad otw.
    \end{cases}
\end{align*}







\begin{lemma}
\label{lem:joint-distr}
   Given a time horizon $T \in \NN$, the joint probability distribution over $(\rn, \rna, \rnb)$ is for all $\cn,\cna, \cnb\in [T] $
   \begin{align*}
       &\prob((\rn=\cn, \rna=\cna, \rnb=\cnb) \\
       &\coloneqq 
        \mathrm{Bin}(\cn; \p, T)\cdot \mathrm{Bin}(\cna; \pa, \cn)\cdot \mathrm{Bin}(\cnb; \pb, T-\cn)
   \end{align*}
\end{lemma}
\begin{proof}
    \begin{align*}
        &\prob(\cn, \cna, \cnb)= \prob(\cn)\cdot \prob(\cna\mid \cn)\cdot \prob(\cnb\mid \cn,\cna) \\
        &= \prob(\cn)\cdot \prob(\cna\mid \cn)\cdot \prob(\cnb\mid \cn) = \\
        & \mathrm{Bin}(\cn; \p, T)\cdot \mathrm{Bin}(\cna; \pa, \cn)\cdot \mathrm{Bin}(\cnb; \pb, T-\cn)
    \end{align*}
\end{proof}


Using Lemma~\ref{lem:joint-distr} we can compute precisely the probability of DP being violated during the finite time horizon. 


\begin{lemma}
Let $T\in \NN$ be a fixed time horizon then
\label{lem:expectation}
   \begin{align*}
       \expe\left(\sdp(\rn, \rna, \rnb)\right) = (\pa - \pb)\cdot (1-\p^T-(1-\p)^T)
   \end{align*}
\end{lemma}
\begin{proof}
    We observe that
       \begin{align*}
       &\expe\left(\sdp(\rn, \rna, \rnb)\right) \\
       &= \sum_{\cn=0}^{T} \prob(\cn) \expe(\sdp(\rn, \rna, \rnb) \mid \cn) \\
       &= \sum_{\cn=1}^{T-1} \prob(\cn)\left( \expe\left( \frac{\rna}{\rn}\middle| \cn\right) - \expe\left( \frac{\rnb}{T-\rn}\middle| \cn\right)\right) \\
   \end{align*}
    We can compute 
    \begin{align*}
        \expe\left( \frac{\rna}{\rn}\middle| \cn\right) &=\frac{1}{\cn} \sum_{\cna=0}^{\cn} \cna \prob(\cna\mid \cn) \\
        &= \frac{ \cn\pa}{\cn} = \pa\\
        \expe\left( \frac{\rnb}{T-\rn}\middle| \cn\right) &=\frac{1}{T-\cn} \sum_{\cnb=0}^{\cn} \cnb \prob(\cnb\mid \cn) \\
        &= \frac{ (T-\cn)\pb}{T-\cn} = \pb
    \end{align*}
    Therefore, we obtain 
           \begin{align*}
       &\expe\left(\sdp(\rn, \rna, \rnb)\right) \\
       &=\sum_{\cn=1}^{T-1} \prob(\cn)\left( \pa -\pb \right) \\
       &=\left( \pa -\pb \right)  \sum_{\cn=1}^{T-1} \prob(\cn) \\
       &= \left( \pa -\pb \right) (1-\p^T-(1-\p)^T)
   \end{align*}
\end{proof}



\begin{lemma}
Let $T\in \NN$ be a fixed time horizon then
\label{lem:expectation-bis}
   \begin{align*}
       \vari\left(\sdp(\rn, \rna, \rnb)\right) = 
   \end{align*}
\end{lemma}
\begin{proof}
    We observe that
   \begin{align*}
       &\vari\left(\sdp(\rn, \rna, \rnb)\right) \\
       &= \expe(\sdp(\rn, \rna, \rnb)^2)- \expe(\sdp(\rn, \rna, \rnb))^2
   \end{align*}
   We know that 
   \begin{align*}
       &\expe(\sdp(\rn, \rna, \rnb))^2 = \left( \pa -\pb \right)^2 (1-\p^T-(1-\p)^T)^2
   \end{align*}
   Furthermore, be definition we obtain
      \begin{align*}
       &\expe(\sdp(\rn, \rna, \rnb)^2) \\
       &= \sum_{\cn=0}^{T} \prob(\cn) \cdot   \expe\left( \left( \frac{\rna}{\rn} - \frac{\rnb}{T-\rn} \right)^2 \middle| \cn\right)  \\
        &= \sum_{\cn=1}^{T-1} \prob(\cn) \cdot   \expe\left( \left( \frac{\rna}{\rn} - \frac{\rnb}{T-\rn} \right)^2 \middle| \cn\right)  \\
   \end{align*}
   We can decompose the expectation into 
   \begin{align*}
       \expe\left(  \frac{\rna^2}{\rn^2} \middle| \cn\right) +  \expe\left(  \frac{\rnb^2}{(T-\rn)^2} \middle| \cn\right) - 2  \expe\left( \frac{\rna}{\rn}\frac{\rnb}{T-\rn}\middle| \cn\right) 
   \end{align*}
   By simple computation we obtain
   \begin{align*}
        &\expe\left(  \frac{\rna^2}{\rn^2} \middle| \cn\right) = \frac{1}{\cn^2} \sum_{\cna=0}^{\cn} \cna^2 \prob(\cna \mid \cn)\\
        &=  \frac{1}{\cn^2}  \expe(\cna^2)\\
         &=  \frac{1}{\cn^2} ( \vari(\cna) + \expe(\cna)^2)\\
          &=  \frac{1}{\cn} \pa(1-\pa) + \pa^2
   \end{align*}
   The same derivation holds for group $b$, i.e., 
     \begin{align*}
        &\expe\left(  \frac{\rnb^2}{T-\rn^2} \middle| \cn\right) = \frac{1}{(T-\cn)^2} \sum_{\cnb=0}^{\cn} \cnb^2 \prob(\cnb \mid \cn)\\
        &=  \frac{1}{(T-\cn)^2}  \expe(\cnb^2)\\
         &=  \frac{1}{(T-\cn)^2} ( \vari(\cnb) + \expe(\cnb)^2)\\
          &=  \frac{1}{(T-\cn)} \pb(1-\pb) + \pb^2
   \end{align*}
   Lastly we compute 
   \begin{align*}
       &\expe\left( \frac{\rna}{\rn}\frac{\rnb}{T-\rn}\middle| \cn\right)  \\
       &=\frac{1}{\cn}\frac{1}{T-\cn}\expe\left( \rna \cdot \rnb \middle| \cn\right)\\
        &=\frac{1}{\cn}\frac{1}{T-\cn}\expe\left( \rna \middle| \cn\right)\cdot\expe\left( \rnb \middle| \cn\right) \\
        &= \frac{1}{\cn}\frac{1}{T-\cn} \cn\pa \cdot (T-\cn)\pb\\
        &= \pa\pb
   \end{align*}
   Putting everything together we obtain
   
\end{proof}







% \begin{lemma}
% \label{lem:unbiased}
%     The empirical analog to SDP is an unbiased estimator, i.e., for every time horizon $T$ we have
%    \begin{align*}
%        \expe\left(\frac{\rna}{\rn} - \frac{\rnb}{T-\rn}\right) = \pa - \pb
%    \end{align*}
%    Moreover, we know that 
%       \begin{align*}
%       \expe\left( \left| \frac{\rna}{\rn} - \frac{\rnb}{T-\rn} \right|\right) \geq \left|\pa - \pb \right| 
%    \end{align*}
%    \KK{Corner case missing.}
% \end{lemma}
% \begin{proof}
%     Observe that 
%     \begin{align*}
%         &\expe\left(\frac{\rna}{\rn}\right) = \sum_{\cn=0}^T\sum_{\cna=0}^T  \frac{\cna}{\cn} \prob(\cn, \cna) \\
%         &=\sum_{\cn=0}^T \frac{1}{\cn} \prob(\cn)  \sum_{\cna=0}^{\cn} \cna  \prob(\cna \mid \cn) \\
%         &= \sum_{\cn=0}^T \frac{1}{\cn} \prob(\cn) \expe(\rna \mid \cn)\\
%         &= \sum_{\cn=0}^T \frac{1}{\cn}\prob(\cn) \pa \cn \\
%         &= \pa \sum_{\cn=1}^T \frac{ \cn}{\cn} \prob(\cn)  \\
%         &=  \pa .
%     \end{align*}
%     Analogue for $\frac{\rnb}{T-\rn}$.
%     The second claim is a direct consequence of Jensen's inequality, i.e., 
%     \begin{align*}
%         \left|\pa - \pb \right| &= \left| \expe\left(\frac{\rna}{\rn} - \frac{\rnb}{T-\rn}\right)  \right|  \\
%         &\leq   \expe\left( \left| \frac{\rna}{\rn} - \frac{\rnb}{T-\rn} \right|\right)
%     \end{align*}
% \end{proof}




\begin{lemma}
\label{lem:variance}
    The variance of the empirical analog to SDP is
    \begin{align*}
        \vari\left(\frac{\rna}{\rn} - \frac{\rnb}{T-\rn} \right)=
    \end{align*}
\end{lemma}
\begin{proof}
    \KK{Corner case}
    We know that we can decompose the variance as follows,
    \begin{align*}
        \vari\left(\frac{\rna}{\rn}\right) + \vari\left(\frac{\rnb}{T-\rn} \right) - 
        2\mathrm{cov}\left(\frac{\rna}{\rn}, \frac{\rnb}{T-\rn}\right)
    \end{align*}
    First
    \begin{align*}
         &\vari\left(\frac{\rna}{\rn}\right) = \expe\left(\frac{\rna^2}{\rn^2}\right) - \expe\left(\frac{\rna}{\rn}\right)^2 \\
         &= \expe\left(\frac{\rna^2}{\rn^2}\right) - \pa^2 \\
        &= \sum_{\cn =0 }^T \prob(\cn) \frac{1}{\cn^2} \expe(\rna^2 \mid \cn)  - \pa^2 \\
        &= \sum_{\cn =0 }^T \prob(\cn) \frac{1}{\cn^2} \left( \cn\pa(1-\pa) + \cn^2\pa^2 \right)  - \pa^2 \\
        &= \pa(1-\pa) \sum_{\cn =0 }^T \prob(\cn) \frac{1}{\cn} +  \pa^2   - \pa^2 \\
         &= \pa(1-\pa) \sum_{\cn =0 }^T \prob(\cn) \frac{1}{\cn} \\
         % &= \pa \sum_{\cn =0 }^T \prob(\cn) \frac{1}{\cn} - \pa^2 \sum_{\cn =0 }^T \prob(\cn) \frac{1}{\cn}  \\
    \end{align*}
    If we assume that DP has an additional $+1$ in the denominator we can exactly express 
    \begin{align*}
        \sum_{\cn =0 }^T \prob(\cn) \frac{1}{\cn+1} = \frac{1-(1-\p)^{T+1}}{(T+1)\p}
    \end{align*}
    then if follows that
    \begin{align*}
        \vari\left(\frac{\rna}{\rn+1}\right) =  \pa(1-\pa) \frac{1-(1-\p)^{T+1}}{(T+1)\p}\\
    \end{align*}
    Second we bound the covariance.
       \begin{align*}
      &\mathrm{cov}\left(\frac{\rna}{\rn}, \frac{\rnb}{T-\rn}\right) 
     \\
     &= \expe\left( \frac{\rna}{\rn} \frac{\rnb}{T-\rn}  \right) -  \expe\left( \frac{\rna}{\rn} \right)\expe\left( \frac{\rnb}{T-\rn}  \right)\\
     &= \expe\left( \frac{\rna}{\rn} \frac{\rnb}{T-\rn}  \right) -  \pa\pb \\
    &= \expe\left( \expe\left( \frac{\rna}{\rn} \frac{\rnb}{T-\rn} \middle| \rn \right) \right) -  \pa\pb \\
     &= \sum_{\cn=0}^T \prob(\cn) \expe\left( \frac{\rna}{\rn} \frac{\rnb}{T-\rn}   \middle| n \right)  -  \pa\pb \\
      &= \sum_{\cn=0}^T \prob(\cn) \expe\left( \frac{\rna}{\rn} \middle|  n\right)  \expe\left( \frac{\rnb}{T-\rn}   \middle|  n \right)  -  \pa\pb \\
      &= \sum_{\cn=0}^T \prob(\cn)\pa\pb - \pa\pb = 0
    \end{align*}
    Third we observe that $T-\rn$ is distributed according to $\mathrm{Bin}(T, 1-p)$. This
    \begin{align*}
        T-\rn= T- \sum_{i=1}^T \rG_i =  \sum_{i=1}^T 1-\rG_i
    \end{align*}
    where $1-\rG_i$ are i.i.d.\ Bernoulli random variables with parameter $(1-\p)$.
    \begin{align*}
         &\vari\left(\frac{\rnb}{T-\rn}\right) = \expe\left(\frac{\rnb^2}{(T-\rn)^2}\right) - \expe\left(\frac{\rnb}{T-\rn}\right)^2 \\
         &= \expe\left(\frac{\rnb^2}{(T-\rn)^2}\right) - \pb^2 \\
         &= \pb(1-\pb) \sum_{\cn =0 }^T \prob(\cn) \frac{1}{T-\cn} \\
         % &= \pa \sum_{\cn =0 }^T \prob(\cn) \frac{1}{\cn} - \pa^2 \sum_{\cn =0 }^T \prob(\cn) \frac{1}{\cn}  \\
    \end{align*}
    Therefore, the variance is 
       \begin{align*}
        \pa(1-\pa) \frac{1-(1-\p)^{T+1}}{(T+1)\p} + \pb(1-\pb) \frac{1-(1-\p)^{T+1}}{(T+1)\p}
    \end{align*}
    \KK{Not correct sort out problem with denominator}
\end{proof}


% 

% Suppose that $p_{1|g}$ is the actual probability of a member of group $g\in\aG$ of being accepted. The real demographic parity is $\DP = |\pa - \pb|$.


==> 87_macros_corner.tex <==
\begin{table}[h]
\caption{Macros cheatsheet}
{\renewcommand{\arraystretch}{1.5} % Adjust the value as needed
\begin{tabular}{lll}
\textbf{Symbol}          & \textbf{Command} & \textbf{Meaning} \\ \hline
$\aF$ & \verb|\aF| & Non-sensitive feature space of the classifier \\ \hline
$\aG$ & \verb|\aG| & Sensitive feature space of the classifier. $\aG = \{a,b\}$ \\ \hline
$\BB$ & \verb|\BB| & Boolean domain in general, $\BB = \{0,1\}$. \\ \hline
$\sagent$ & \verb|\sagent| & An ML classifier, $\sagent\colon \aG\times\aF \to \BB\times \mathbb{R}_{\geq 0}$. \\ \hline
$\prob$ & \verb|\prob| & Probability. Also for probability distribution functions. \\ \hline

$\distrset()$ & \verb|\distrset| & Probability distribution. For example, $P_\sagent \in \distrset(\aX)$. \FC{Shouldn't this be $\prob_\sagent \in \distrset(\aX)$ ?} \\ \hline
$\aX$ & \verb|\aX|         &  Input space, of the shield, $\aX \coloneqq \support(P_\sagent) \subseteq \aG\times \BB\times\RR_{\geq 0}$      \\ \hline
$\aY$  & \verb|\aY|         & Decision space of the shield, $\aY = \{0,1\}$. \\   \hline
$\indicator{}$ & \verb|\indicator{}| & Indicator function, $\indicator{b} = 1$ if $b$ is true, and $0$ if $b$ is false. \\ \hline
$\sshield$ & \verb|\sshield| & A shield, $\sshield\colon \left(\aX\times\aY\right)^*\times \aX \to \aY$  \\ \hline
$\sShield$ & \verb|\sShield| & The set of all shields \\ \hline
$\cost$ & \verb|\cost| & Cost function, $\cost(\tau;s) \coloneqq \sum_{i=1}^s c_i\cdot\indicator{r_i\neq y_i}.$ \\ \hline
$\DP$ & \verb|\DP| & Demographic parity, $\DP(\tau) = \left| \frac{n_{a1}}{n_a} - \frac{n_{b1}}{n_b} \right|$. \\ \hline
$\sShieldFeas$ & \verb|\sShieldFeas| & Set of fairness enforcing shields, $\sShieldFeas^{t,\tau}$ when a prefix trace $\tau$ and \\ &  & time horizon $t$ is specified. \\ \hline
$\costset$ & \verb|\costset| & Set of values that the cost can take. $\costset$ is finite and $\costset \subseteq \RR_{\geq 0}$. \\ \hline
$\Trfeas$ & \verb|\Trfeas| & Set of feasible traces
$\Trfeas^{t}_{\sagent,\sshield} =
\{ \tau \in (\aX\times\aY)^t \:|\: \prob(\tau; P_\sagent, \sshield) > 0 \}$ \\ \hline
$\AccRate{g}{\tau}$ & \verb|\AccRate{g}{\tau}| & Acceptance rate, given a trace $\tau$ and group $g$, $\AccRate{g}{\tau} = \frac{\sum_i \indicator{y_i=1\land g_i=g}}{\sum_i\indicator{g_i=g}}$ \\ \hline
$\Trbalance$ & \verb|\Trbalance| & Set of balanced traces, $\Trbalance_N^t$ is the set of traces of length $t$ with at least \\ & & $N$ individuals of each group. \\ \hline
$\costset$ & \verb|\costset| & Cost set \\ \hline
$\popdistr$ & \verb|\popdistr| & Underlying distribution of the population \\ \hline
$\traindata$ & \verb|\traindata| & Training data for cost alignment \\ \hline
$\FinShield$ & \verb|\FinShield| & Finite horizon shield, "normal" shield \\ \hline
$\StaticDP$ & \verb|\StaticDP| & Static DP shield, aka "naive" shield \\ \hline
$\StaticBAR$ & \verb|\StaticBAR| & Static Bounded Acceptance Rates shield \\ \hline
$\Dyn$ & \verb|\Dyn| & Dynamic shield, aka "buffered" shield
\end{tabular}}
\end{table}




% \newcommand{\FinShield}{\textsf{FinHzn}\xspace}
% \newcommand{\StaticDP}{\textsf{Static-DP}\xspace}
% \newcommand{\StaticBAR}{\textsf{Static-BAR}\xspace}
% \newcommand{\Dyn}{\textsf{Dynamic}\xspace}
% \newcommand{\BAR}{\text{BAR}\xspace}
